Reflection-dominated Compton-thick AGN Candidates in the SRG/eROSITA Lockman Hole Survey

We search for reflection-dominated Compton-thick active galactic nuclei (CT AGN) candidates in the Lockman Hole region using the data of SRG/eROSITA Lockman Hole survey. We selected sources with anomalously hard photon indices in the $0.3 - 8.0$ keV band, untypical for type I AGN. In particular, we required that the upper end of the $90\%$ error interval did not exceed a fiducial boundary of $\Gamma=1.3$. We found 291 sources which constitute a rare subpopulation among extragalactic X-ray sources detected by eROSITA in the Lockman Hole field, $\approx 5\%$. These sources constitute the eROSITA sample of CT AGN candidates in the Lockman Hole field. We further divide the sources into three categories depending on the availability of reliable redshift and statistically significant detection of intrinsic absorption. We present two catalogues: the bright sample (37 sources) and the faint one (254). We estimate the fraction and sky density of reflection-dominated CT AGN candidates. We show examples of individual spectra and use stacking analysis to search for possible redshift evolution of their properties with redshift. We analyse combined eROSITA spectra of bright sources of different categories with a physically motivated spectral model UXCLUMPY and find them fully consistent with the fits to the about $\sim 1$ Msec XMM-Newton data for one of our reflection-dominated CT candidates, Type 2 galaxy $\text{SRGe J105348.6+573032}$. The catalogues of CT AGN candidates could be a good starting point for planning future studies and follow-ups at all wavelengths.

==> tables/scheme.tex <==
\begin{tikzpicture}[
    level/.style={sibling distance=3.5cm, level distance=2cm}
    ]
  % Define the nodes
  \node {Initial sample (6528)}
    child {node {$\Gamma$ upper limit < 1.3}
        child {node[align=center] {Is reliable redshift \\available?}
            child {node[align=center] {Is significant \\intrinsic $\nh$ detected?}
                child {node[align=center] {Mildly obscured \\ AGN candidates, \\ Category 2}
                edge from parent node[left, xshift=-1mm, yshift=1mm] {\small \textbf{Yes (49)}}
                }
                child {node[align=center] {Reflection-dominated \\CT AGN candidates,\\ Category 1}
                edge from parent node[right, xshift=2mm, yshift=-1mm] {\small \textbf{No (81)}}
                }
                edge from parent node[left, xshift=-1mm, yshift=1mm] {\small \textbf{Yes (130)}}
            }
        child {node[align=center] {No redshift avaliable,\\ Category 3 candidates}
        edge from parent node[right, xshift=1mm, yshift=1mm] {\small \textbf{No (161)}}
        }
        }};
\end{tikzpicture}
